Learning to Acquire Information

We consider the problem of diagnosis where a set of simple observations are used to infer a potentially complex hidden hypothesis. Finding the optimal subset of observations is intractable in general, thus we focus on the problem of active diagnosis, where the agent selects the next most-informative observation based on the results of previous observations. We show that under the assumption of uniform observation entropy, one can build an implication model which directly predicts the outcome of the potential next observation conditioned on the results of past observations, and selects the observation with the maximum entropy. This approach enjoys reduced computation complexity by bypassing the complicated hypothesis space, and can be trained on observation data alone, learning how to query without knowledge of the hidden hypothesis.

==> decision.tex <==
\section{Active Diagnosis as Decision Tree}

One useful view of active diagnosis is as a decision tree, where each decision node in the tree correspond to a possible observation, and the hypothesis are leaves. At each time-step, the decision tree informs one which next observation to choose based on the outcomes of all previous observations. This information of previous observations is encoded as a path from the root node of the decision tree to the current decision node. To determine the exact hypothesis with as few observations as possible amounts to construct a decision tree that is short in height. In practice, maintaining such a decision tree data-structure is infeasible as it would require exponentially many decision nodes proportional to the number of observations. Therefore, instead of constructing and storing a pre-computed decision tree, one can view most active diagnosis algorithms as a lazy construction of decision trees on the fly, which computes the optimal next observation in run-time.

In this section we describe our approach as a construction of a decision tree, and compare it against previous approaches.

\subsection{Problem Definition}
Let the hidden hypothesis be $S$, a random variable that can take on values $s \in dom(S)$, which is responsible for generating a finite set of observations $O_1 \dots O_N$, where each observations can take on values $o \in dom(O)$. For this section, we will assume each hypothesis $s \in S$ has equal probability, and that each observation is a binary observation of either $True$ or $False$ value. We also assume each observation to be unambiguous, that is to say, for any $s \in S$ and $O_i$, the observation is either $True$ or $False$ with probability $1$.

Let $O^{-} = \{ O^1=o^1 \dots O^K=o^K \}$ denotes the outcomes of some $K$ observations, note that since the observations are unambiguous, this induces a consistent subset on the hypothesis space where:

\begin{equation*}
\begin{split}
	S_{\big| O^{-}} = \{s \in S | consistent(s, O^{-}) \} 
\end{split}
\end{equation*}

Here, consistent means the hypothesis $s$ do not generate an observation that is contradictory to the outcomes in $O^{-}$.

Let's consider the family of set of observations where the consistent subset is non-empty:

\begin{equation*}
\begin{split}
	\{O^{-} | S_{\big| O^{-}} \neq \{\} \} 
\end{split}
\end{equation*}







==> exp_mnist.tex <==
\subsection{MNIST}

MNIST is a simple image classification dataset consists of 60000 training examples and 10000 testing examples. Given an image, standard image classification schemes such as convolutional neural network with dropout (Srivastava 2014) can achieve an error rate of 0.73\%. In this work we consider a different problem: Is it possible to accurately classify the image by intelligently choose a subset of the pixels? 

The same problem was considered by (Mnih, 2014), where the MNIST image was being classified after observing a number of 8 by 8 pixel patches, called glimpses. The problem was phrased as an instance of reinforcement learning, where the agent sequentially decide for a number of steps the location for the next glimpse, and as the final action output the predicted label of the image. They are able to achieve an error rate of 3.79\% with 2 glimpses, and an error rate of 1.07\% with 7 glimpses. One drawback of this approach is the requirement of a large number of labeled instances to train the glimpse network, as the reward signal for taking a good glimpse ultimately originates from the last action of the network, which predicts the true label. By contrast, our observation collection algorithm OC depends on the implication model $Pr(O^{K+1} | O^{-})$, which require data only about the image pixels and not the image labels. This is an important advantage as our OC algorithm can be trained from unlabeled data alone.

We setup our experiment as follows: The training data is restricted to contain only 1000 labeled instances, and 59000 unlabeled instances, pre-processed to be black-white rather than grey-scale. From the labeled instance we train a simple fully-connected 2 layer neural network (the same architecture used by Mnih, 2016) for the standard classification task, which only works on a fully observed image. Then, we train our implication model required by the OC on the unlabeled data. At test time, we use OC to collect a set of observations by querying for the most informative pixel coordinates, and ``completes'' these sparse pixel observation to a full image by outputting its belief space. This completed image is then run through the classifier to give a label prediction. Overall, our approach uses OC which is trained from a large number of unlabeled data (60000), and a classifier which is trained from a small number of labeled data (1000).

Figure \ref{fig:mnist_belief} shows the belief space of the OC algorithm at various number of observed pixels, note with only 11 observations it generates a belief space that is fairly consistent with the underlying hypothesis (the number 9).

\begin{figure}[!ht]
  \centering
    \includegraphics[width=8.2cm,height=7cm,keepaspectratio]{figs/mnist_belief.png}
  \caption{Belief space of the OC algorithm on different numbers of observations}
    \label{fig:mnist_belief}
\end{figure}

We compare our approach with the following baselines: The \textbf{ran\_oc} is like OC except it picks its observations at random rather than querying for the most informative pixel. The restricted  OC \textbf{res\_oc} trains the implication model used by OC on the 1000 labeled data which the classifier is also trained on alone. The full observable baseline \textbf{full} uses the classifier directly on the full image, assuming all pixel values are available.

Figure (run it)

==> formats.tex <==

\section{GENERAL FORMATTING INSTRUCTIONS}

Papers are in 2 columns with the overall line width of 6.75~inches
(41~picas).  Each column is 3.25~inches wide (19.5~picas).  The space
between the columns is .25~inches wide (1.5~picas).  The left margin
is 1~inch (6~picas).  Use 10~point type with a vertical spacing of
11~points.  Times Roman is the preferred typeface throughout.

Paper title is 16~point, caps/lc, bold, centered between 2~horizontal
rules.  Top rule is 4~points thick and bottom rule is 1~point thick.
Allow 1/4~inch space above and below title to rules.

Reviewing is double-blind, so do not include author names, affiliations, or any
other identifying information in the original submission.  If you include urls
to supplementary material, make sure the urls also do not disclose your identity.

After a paper is accepted, for the camera-ready submission, Authors' names are
centered, initial caps.  The lead author's name is to be listed first
(left-most), and the Co-authors' names (if different address) are set to
follow.  If only one co-author, center both the author and co-author,
side-by-side.

One-half line space between paragraphs, with no indent.

\section{FIRST LEVEL HEADINGS}

First level headings are all caps, flush left, bold and in point size
12. One line space before the first level heading and 1/2~line space
after the first level heading.

\subsection{SECOND LEVEL HEADING}

Second level headings must be flush left, all caps, bold and in point
size 10. One line space before the second level heading and 1/2~line
space after the second level heading.

\subsubsection{Third Level Heading}

Third level headings must be flush left, initial caps, bold, and in
point size 10.  One line space before the third level heading and
1/2~line space after the third level heading.

\vskip .5pc
Fourth Level Heading

Fourth level headings must be flush left and initial caps.
One line space before the fourth level heading and 1/2~line space
after the fourth level heading.

\subsection{CITATIONS, FIGURES, REFERENCES}


\subsubsection{Citations in Text}

Citations within the text should include the author's last name and
year, e.g., (Cheesman, 1985). Reference style should follow the style
that you are used to using, as long as the citation style is
consistent.

For the original submission, take care not to reveal the authors' identity through
the manner in which one's own previous work is cited.  For example, writing
``In (Bovik, 1970), we studied the problem of AI'' would be inappropriate, as
it reveals the author's identity.  Instead, write ``(Bovik, 1970) studied the
problem of AI.''

\subsubsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first
footnote} in the text. Use 8 point type for footnotes.  Place the
footnotes at the bottom of the page on which they appear.  Precede the
footnote with a 0.5 point horizontal rule 1~inch (6~picas)
long.\footnote{Sample of the second footnote}

\subsubsection{Figures}

All artwork must be centered, neat, clean, and legible. Figure number
and caption always appear below the figure.  Leave 2 line spaces
between the figure and the caption. The figure caption is initial caps
and each figure numbered consecutively.

Make sure that the figure caption does not get separated from the
figure. Leave extra white space at the bottom of the page rather than
splitting the figure and figure caption.
\begin{figure}[h]
\vspace{1in}
\caption{Sample Figure Caption}
\end{figure}

\subsubsection{Tables}

All tables must be centered, neat, clean, and legible. Table number
and title always appear above the table.  See
Table~\ref{sample-table}.

One line space before the table title, one line space after the table
title, and one line space after the table. The table title must be
initial caps and each table numbered consecutively.

\begin{table}[h]
\caption{Sample Table Title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION} \\
\hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\newpage


==> stash.tex <==
The problem of active diagnosis is defined as finding a subset of observations $\{O^1 \dots O^M\}$ such that the mutual information between the subset and the hidden hypothesis is maximized.

\[
	\argmax_{\{O^1 \dots O^M\} \in \{O_1 \dots O_N\}^M} I(S, \{O^1 \dots O^M\})
\]

Finding the optimal subset is known to be intractable in practice (Littman, 1998), and the standard approach is to adopt a greedy strategy that aims to maximize mutual information 1 item at a time (Golovin, 2011): Given a set (of potentially empty) current observations $\{ O^1=o^1 \dots O^K=o^K \}$ we wish to choose an additional observation $O^{K+1}$ among the set of observations $O_1 \dots O_N$ that maximizes mutual information between it and the hidden hypothesis: 

\[
	\argmax_{O^{K+1} \in \{O_1 \dots O_N\}} I(S, O^{K+1} | O^1=o^1 \dots O^K=o^K)
\]

For brevity, let's write the past observations as $O^{-} := \{O^1=o^1 \dots O^K=o^K\}$ 

One can evaluate mutual information directly as follows:

\begin{equation*}
\begin{split}
	I(S, O^{K+1} | O^{-}) = \sum_{o^{k+1}} \sum_{s} & log P(O^{k+1} = o, S = s | O^{-} ) \\
    & \frac{P(O^{k+1} = o, S = s | O^{-} )}
    {P(O^{k+1} = o| O^{-} ) P(S = s | O^{-} ) }
\end{split}
\end{equation*}

However, if $|dom(S)|$ is sufficiently large this computation becomes infeasible. 

However, one can decompose mutual information as a difference of entropy in two ways:

\begin{equation}
\begin{split}
	& \argmax_{O^{K+1} \in \{O_1 \dots O_N\}} I(S, O^{K+1} | O^{-}) \\
    =& \argmax_{O^{K+1} \in \{O_1 \dots O_N\}} H(S | O^{-}) - H(S | O^{K+1}, O^{:
}) \\
    =& \argmax_{O^{K+1} \in \{O_1 \dots O_N\}} H(O^{K+1} | O^{-}) - H(O^{K+1} | S, O^{-})
\end{split}
\end{equation}

We will now analyze the properties of each decomposition and show why the second decomposition is easier to model under the right assumptions.



\subsection{Hypothesis Centric Decomposition}

Let us consider the first decomposition:



Here, $H(S | O^{-}) $ is a constant as it does not depend on $O'$, thus the problem reduces to:

\begin{equation}
\begin{split}
&\argmax_{O' \in \{O_1 \dots O_N\}} I(S, O' | O^{-}) \\
=& \argmin_{O' \in \{O_1 \dots O_N\}} H(S | O', O^{-}) \\
=& \argmin_{O' \in \{O_1 \dots O_N\}} \sum_{o} Pr(O'=o | O^{-}) \\
 & ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~H(S | O'=o, O^{-})
\end{split}
\end{equation}

This objective function of reducing entropy on the hypothesis space is the approach used by (Rish, 2004), (Bellala, 2013), and (Zheng, 2012).

To compute $Pr(O'=o | O^{-})$:
\begin{equation*}
\begin{split}
& Pr(O'=o | O^{-}) \\
=& \sum_{s} Pr(S=s | O^{-}) Pr(O'=o | S=s, O^{-}) \\
=& \sum_{s} Pr(S=s | O^{-}) Pr(O'=o | S=s) \\
\propto & \sum_{s} (Pr(S=s) \prod_{k} Pr(O^k = o^k | S=s))  \\
 &~~~~~~~~Pr(O'=o | S=s)
\end{split}
\end{equation*}

This computation would take $O(dom(S)K)$ operations

To compute $H(S | O'=o, O^{-})$:
\begin{equation*}
\begin{split}
&H(S | O'=o, O^{-}) \\
=& \sum_{s} Pr(S=s | O'=o, O^{-}) \\
&~~~~~~~~logPr(S=s | O'=o, O^{-}) 
\end{split}
\end{equation*}

Where $Pr(S=s | O'=o, O^{-})$ can be computed by:
\begin{equation*}
\begin{split}
& Pr(S=s | O'=o, O^{-}) \\
\propto & \sum_{s} Pr(S=s) \prod_{k} Pr(O^k = o^k | S=s) \\ 
&~~~~~~~~Pr(O'=o| S=s) \\
\end{split}
\end{equation*}

This computation would take $O(dom(S)K)$ operations as well. Overall finding the most informative observation would take O(NKdom(O)dom(S)) operations. The culprit here is $dom(S)$, which can be complex if one is working over a complex hypothesis domain, and computation over $dom(S)$ cannot be avoided as one needs to compute the entropy term $H(S | O'=o, O^{-})$

\subsection{Observation Centric Decomposition}

Consider the second decomposition:
\begin{equation}
\begin{split}
	& \argmax_{O' \in \{O_1 \dots O_N\}} I(S, O' | O^{-}) \\
    =& \argmax_{O' \in \{O_1 \dots O_N\}} H(O' | O^{-}) - H(O' | S, O^{-})
\end{split}
\end{equation}

At first glance this decomposition is no less difficult than the first, as both entropy terms depends on $O'$, which would suggest that both needs to be computed. 

We now introduce the assumption of uniform observation entropy, which would allow us to greatly simplify the computation under this decomposition.

\paragraph{Uniform Observation Entropy} The property of uniform observation entropy hold if, when a hypothesis is given $S=s$, the entropy for each observation class $O_i$ are equal: 
\begin{equation}
\begin{split}
	\forall i,j \in \{1 \dots N\}^2: H(O_i | S=s) = H(O_j | S=s)
\end{split}
\end{equation}
This is a reasonable assumption as one can often assume the noise from the observation usually arise from a noisy channel, which corrupts the noiseless observations equally regardless of which observation. In the extreme case the observations have $0$ entropy if they can be made without noise.

Thus, $H(O' | S, O^{-})$ can be computed by:
\begin{equation}
\begin{split}
&H(O' | S, O^{-}) \\
=& \sum_{s} Pr(S=s|O^{-}) H(O^{k+1} | S=s, O^{-}) \\
=& \sum_{s} Pr(S=s|O^{-}) H(O^{k+1} | S=s)
\end{split}
\end{equation}

Note:
\begin{itemize}
\item The term $Pr(S=s|O^{-})$ is a constant with respect to $O'$
\item Under the assumption of uniform observation entropy, $H(O^{k+1} | S=s) $ is also a constant for any choice of $O' \in \{O_1 \dots O_N\}$
\end{itemize} 

Thus, under our assumptions $H(O' | S, O^{-})$ becomes a constant, and the problem reduces to:
\begin{equation}
\begin{split}
	& \argmax_{O' \in \{O_1 \dots O_N\}} I(S, O' | O^{-}) \\
    =& \argmax_{O' \in \{O_1 \dots O_N\}} H(O' | O^{-}) 
\end{split}
\end{equation}

The computation of $H(O' | O^{-})$ would take $O(dom(O)dom(S)K)$ operations, and the overall computation complexity is $O(NKdom(O)dom(S))$ operations, which is no better than the first decomposition.

However, note that the complexity of $dom(S)$ only arises in trying to compute $Pr(O' | O^{-})$, which, if we were to model this probability directly, would obtain a complexity of $O(NKdom(O)c)$ operations, where $c$ is a constant relative to the size of our modeling parameters computing $Pr(O' | O^{-})$.

We call the modeling of $Pr(O' | O^{-})$ an \emph{implication model} because it is attempting to deduce the outcome of a future observation based on a set of past observations. We will describe how to train this model in the next section. 

We would like to remark that one can consider the approaches by (Joshi, 2009), (Tong, 2001) and (Lewis, 1994) as a way of approximating $H(O' | O^{-})$. Instead of computing over all possible hypothesis in $dom(S)$, these approaches computes the most likely hypothesis:
\begin{equation*}
\begin{split}
	s^* = \argmax_{s \in dom(S)} Pr(S=s|O^{-})
\end{split}
\end{equation*}

then use the most likely hypothesis $s^*$ to query for observations that are maximally confusing to it
\begin{equation*}
\begin{split}
	O' = \argmax_{O' \in \{O_1 \dots O_N\}} H(O'|S=s^*)
\end{split}
\end{equation*}

(Holub, 2008) uses an approach that is most similar to ours: They attempt to minimize the conditional entropy of the unlabeled data conditioned on the labeled data, which is equivalent to our approach of maximizing the conditional entropy of the chosen observation conditioned on past observations. The difference is that in their approach the conditional entropy is approximated by a committee of classifiers/hypothesis, while our approach attempt to compute the conditional entropy directly.


\subsection{Our Algorithm}

Our algorithm is divided into 2 parts, observation collection and hypothesis delivery. In observation collection, a set of observations are adaptively chosen at each time step by maximizing the entropy $H(O' | O^{-})$ until a budgeted limit. These observations are then used to deliver a hypothesis by a separate algorithm.

\begin{algorithm}
\kwRequire{$Pr(O' | O^{-})$}
\kwRequire{$query_s(O)$}
 $O^{-}$ = \{\} \\
 \While{size($O^{-}$) $\le$ Budget}{
  O = $\argmax_{O' \in \{O_1 \dots O_N\}} H(O' | O^{-}) $ \\
  o = $query_s(O)$ \\
  $O^{-}$ $\leftarrow$ $O^{-}$ $\cup$ \{O=o\} \\
 }
 \kwReturn{$O^{-}$}
 \caption{Observation Collection}
\end{algorithm}

Here, $query$ is a function which returns the value for an observation given a hidden hypothesis $s$.

The inference for the hidden hypothesis is performed in a problem specific manner: For some problem it is appropriate to train a classifier that classifies the hidden hypothesis, for other problems one can compute the hidden hypothesis directly from the observations. We will discuss the hypothesis inference in detail in the experiment section. We would like to remark that our scheme is unique in that the observation collection algorithm is completely decoupled from the hypothesis delivery algorithm, this decoupling would allow one to explore different hypothesis delivery algorithms with the guarantee that the observations being  used to deliver the hypothesis are well chosen. 

The keystone of our scheme is modeling the probability $Pr(O' | O^{-})$, which is used to compute the entropy term $H(O' | O^{-})$ in the observation collection algorithm. In the next section we describe in detail how to model and train this distribution.

% \begin{algorithm}
%  \KwData{this text}
%  \KwResult{how to write algorithm with \LaTeX2e }
%  initialization\;
%  \While{not at end of this document}{
%   read current\;
%   \eIf{understand}{
%    go to next section\;
%    current section becomes this one\;
%    }{
%    go back to the beginning of current section\;
%   }
%  }
%  \caption{How to write algorithms}
% \end{algorithm}








